A Bayesian Time-Varying Autoregressive Model for Improved Short- and Long-Term Prediction

Motivated by the application to German interest rates, we propose a timevarying autoregressive model for short and long term prediction of time series that exhibit a temporary non-stationary behavior but are assumed to mean revert in the long run. We use a Bayesian formulation to incorporate prior assumptions on the mean reverting process in the model and thereby regularize predictions in the far future. We use MCMC-based inference by deriving relevant full conditional distributions and employ a Metropolis-Hastings within Gibbs Sampler approach to sample from the posterior (predictive) distribution. In combining data-driven short term predictions with long term distribution assumptions our model is competitive to the existing methods in the short horizon while yielding reasonable predictions in the long run. We apply our model to interest rate data and contrast the forecasting performance to the one of a 2-Additive-Factor Gaussian model as well as to the predictions of a dynamic Nelson-Siegel model.

==> TitlepageAndAbstract.tex <==
\title{A Bayesian Time-Varying Autoregressive Model for Improved Short- and Long-Term Prediction}
%\subtitle{Christoph Berninger, Almond St\"{o}cker, David R\"{u}gamer}
\author{Christoph Berninger$^1$ \and Almond St\"{o}cker$^2$ \and David R\"{u}gamer$^1$}
\date{%
    \begin{small}
    $^1$Department of Statistics, LMU München\\%
    $^2$ School of Business and Economics, Humboldt University of Berlin%\\[2ex]%
    \end{small}
    % \today
}
\maketitle

\section*{Abstract}

Motivated by the application to German interest rates, we propose a time-varying autoregressive model for short and long term prediction of time series that exhibit a temporary non-stationary behavior but are assumed to mean revert in the long run. We use a Bayesian formulation to incorporate prior assumptions on the mean reverting process in the model and thereby regularize predictions in the far future. We use MCMC-based inference by deriving relevant full conditional distributions and employ a Metropolis-Hastings within Gibbs Sampler approach to sample from the posterior (predictive) distribution. In combining data-driven short term predictions with long term distribution assumptions our model is competitive to the existing methods in the short horizon while yielding reasonable predictions in the long run. We apply our model to interest rate data and contrast the forecasting performance to the one of a 2-Additive-Factor Gaussian model as well as to the predictions of a dynamic Nelson-Siegel model.

